The Marco Polo Problem: A Combinatorial Approach to Geometric Localization

We introduce and study the Marco Polo problem, which is a combinatorial approach to geometric localization. In this problem, we are told there are one or more points of interest (POIs) within distance $n$ of the origin that we wish to localize. Given a mobile search point, $\Delta$, that is initially at the origin, a localization algorithm is a strategy to move $\Delta$ to be within a distance of $1$ of a POI. In the combinatorial localization problem we study, the only tool we can use is reminiscent of the children's game, "Marco Polo," in that $\Delta$ can issue a probe signal out a specified distance, $d$, and the search algorithm learns whether or not there is a POI within distance $d$ of $\Delta$. For example, we could imagine that POIs are one or more hikers lost in a forest and we need to design a search-and-rescue (SAR) strategy to find them using radio signal probes to a response device that hikers carry. Unlike other known localization algorithms, probe responses do not inform our search algorithm of the direction or distance to a POI. The optimization problem is to minimize the number of probes and/or POI responses, as well as possibly minimizing the distance traveled by $\Delta$. We describe a number of efficient combinatorial Marco Polo localization strategies and we analyze each one in terms of the size, $n$, of the search domain. Moreover, we derive strong bounds for the constant factors for the search costs for our algorithms, which in some cases involve computer-assisted proofs. We also show how to extend these strategies to find all POIs using a simple, memoryless search algorithm, traveling a distance that is $\mathcal{O}(\log{k})$-competitive with the optimal traveling salesperson (TSP) tour for $k$ POIs.

==> assumptions.tex <==
\subsubsection{Simple Case: Exactly One POI at Distance at most~\texorpdfstring{$n$}{n}}
\label{sec:bad}
As a warm up for our more interesting results, let us begin
with a simple (but admittedly unrealistic) scenario,
where there is exactly one POI within distance~$n$ of the origin
and we can perform arbitrarily large probes.
In this case, where
we allow unbounded probe distances,
we can find the sole POI using two
binary searches, one in each dimension.
We place $\Delta$ at a very large distance from the origin, such that the
intersection for the probe with the original search region is nearly a
straight line,
and perform one binary search using $\lceil \log{n} \rceil + 1$ probes to find a
region of width at most 1 in the first dimension.
We then perform a similar binary search placing $\Delta$ in an orthogonal
direction to find the POI in the second dimension.
We are left with a region of side length 1, which is fully contained
within a single, final, radius-1 probe.
This solution thus
uses $2 \lceil \log{n} \rceil + \mathcal{O}(1)$ probes,
but it relies on $\Delta$ traveling very far away and at high
altitude and the tracking device to have very strong signal strength,
which are not reasonable assumptions.
This can be improved somewhat
by restricting the probe distance to $n$,
as we explore in an appendix, but
this ``simple'' solution still requires large
probes and high signal strength for the tracking device.
Because of the drawbacks of this ``simple'' solution,
for the remainder
of paper we make two important assumptions:
\begin{itemize}
\item
The maximum allowed probe distance, $d$, is $n$.
% (ii) $\Delta$ is restricted to the original search area, and
\item
There may be multiple POIs,
either within the initial search region of radius $n$ or slightly outside of it.
\end{itemize}


==> find-all-mst.tex <==
\subsection{Reducing the Number of Probes}

While our stateless search algorithm achieves competitive results with regards
to distance traveled, while being very simple and practical, it may still be of
interest to determine exactly how much improvement can be made 

